On numerical inverse scattering for the Korteweg-de Vries equation with discontinuous step-like data

We present a method to compute dispersive shock wave solutions of the Korteweg-de Vries equation that emerge from initial data with step-like boundary conditions at infinity. We derive two different Riemann-Hilbert problems associated with the inverse scattering transform for the classical Schr\"odinger operator with possibly discontinuous, step-like potentials and develop relevant theory to ensure unique solvability of these problems. We then numerically implement the Deift-Zhou method of nonlinear steepest descent to compute the solution of the Cauchy problem for small times and in two asymptotic regions. Our method applies to continuous and discontinuous data.

==> y.tex <==

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:

